Can We Remove the Ground? Obstacle-aware Point Cloud Compression for Remote Object Detection

Efficient point cloud (PC) compression is crucial for streaming applications, such as augmented reality and cooperative perception. Classic PC compression techniques encode all the points in a frame. Tailoring compression towards perception tasks at the receiver side, we ask the question, "Can we remove the ground points during transmission without sacrificing the detection performance?" Our study reveals a strong dependency on the ground from state-of-the-art (SOTA) 3D object detection models, especially on those points below and around the object. In this work, we propose a lightweight obstacle-aware Pillar-based Ground Removal (PGR) algorithm. PGR filters out ground points that do not provide context to object recognition, significantly improving compression ratio without sacrificing the receiver side perception performance. Not using heavy object detection or semantic segmentation models, PGR is light-weight, highly parallelizable, and effective. Our evaluations on KITTI and Waymo Open Dataset show that SOTA detection models work equally well with PGR removing 20-30% of the points, with a speeding of 86 FPS.

==> figlatex/ablation_fig.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/evaluation/second_kitti_ablation.pdf}
  \caption{Ablation study on restoration phase of PGR: PVT-SSD performance (mAP) versus bit per point (bpp) on KITTI.}
\label{fig:comp_ablation}
\end{figure*}

==> figlatex/other-gp-comparison.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/evaluation/second_comparison_no_raw.pdf}
    \caption{Comparison between \ourname and GnDNet \cite{paigwar2020gndnet}, PolarNet \cite{zhang2020polarnet}, and patchwork++ \cite{patchword}: PVT-SSD  performance (mAP) versus bits per point (bpp) on KITTI.}
    \vspace{-3mm}
\label{fig:comp}
\end{figure*}
